ARBERT & MARBERT: Deep Bidirectional Transformers for Arabic

Pre-trained language models (LMs) are currently integral to many natural language processing systems. Although multilingual LMs were also introduced to serve many languages, these have limitations such as being costly at inference time and the size and diversity of non-English data involved in their pre-training. We remedy these issues for a collection of diverse Arabic varieties by introducing two powerful deep bidirectional transformer-based models, ARBERT and MARBERT. To evaluate our models, we also introduce ARLUE, a new benchmark for multi-dialectal Arabic language understanding evaluation. ARLUE is built using 42 datasets targeting six different task clusters, allowing us to offer a series of standardized experiments under rich conditions. When fine-tuned on ARLUE, our models collectively achieve new state-of-the-art results across the majority of tasks (37 out of 48 classification tasks, on the 42 datasets). Our best model acquires the highest ARLUE score (77.40) across all six task clusters, outperforming all other models including XLM-R Large (~ 3.4 x larger size). Our models are publicly available at https://github.com/UBC-NLP/marbert and ARLUE will be released through the same repository.

==> ARBERT_data.tex <==
% #####################################
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[ht]
\centering
\small
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{lcHr}
\hline
\textbf{Source}                          & \textbf{Size}  & \textbf{Sentences} & \textbf{Tokens} \\ \hline
Books (Hindawi)      & $650$MB                   & $2.3$M            & $72.5$M                                 \\
El-Khair & $16$GB      & $42$M           & $1.6$B                              \\

Gigawords    & $10$GB                    & $67.4$M           & $1.1$B                              \\

OSIAN     & $2.8$GB                   & $12$M           & $292.6$M                                \\

OSCAR-MSA        & $31$GB                    & $67.3$M           & $3.4$B          \\
OSCAR-Egyptian      &$32$MB & $101.9$M              & $3.8$M                                  \\
Wiki     & $1.4$GB                   & $12.5$M           & $156.5$M                                \\\hline
\textbf{Total}                           & \textbf{$\bf 61$GB} & \textbf{$ \bf 203.5$M}                      & \textbf{$\bf 6.5$}B        \\ 

\hline

\end{tabular}%
}
\caption{\ourmodel~'s pre-train resources.}
\label{tab:ARABERT_data}
\end{table}
% ###################################

==> discussion.tex <==
\section{General Discussion}\label{sec:experiment}




==> evaluation.tex <==
\section{Experimental Setup and Results}\label{sec:experiment}

This section shows the experimental setting and the performance of our
models by evaluating them on Arabic NLP downstream tasks.
% \input{AraBERT++/comp_arabert}
% \input{AraBERT++/ADI}
\subsection{Fine-tuning Setup}
% \subsubsection{Pre-training}
% We use the same network architecture as mBERT (12-layer, 768-hidden, 12-heads, 110M parameters) ~\cite{devlin2018bert} and used the original implementation of BERT on TensorFlow was used~\footnote{BERT Implementation:~\url{https://github.com/google-research/bert}} and we used the free access to cloud TPUs from TensorFlow Research Cloud (TFRC) to train \ourmodel. The AraBERT model is trained on 8 TPUs (v2.8)~\footnote{TFRC:~\url{https://www.tensorflow.org/tfrc}}. We train \ourmodel on 100K wordPiece vocabulary, for 16 epochs with a batch size of 256 and a maximum sequence length of 128. Training took 14 days on 8 Google Cloud TPUs.\\
% \subsubsection{Fine-tuning}
We slightly normalize the text as remove Arabic diacritics , replace hyperlinks and user mentions with URL and USER respectively. For Twitter hashtags, we removed hash sign and replace underscore with space. We use the splits provided by the dataset’s authors when available and the standard $80\%$ and $20\% $ when not. We fine-tuning the downstream tasks on  AraBERT, mBERT, XLM-R$_{bsea}$, XLM-R$_{large}$, and our proposed models (\ourmodel~and \newmodel) with the same setting. We fine-tuning the models for $25$ epochs using $256$ sequence length and $32$ batch size.  We use $2$-$e^6$  as learning rate on text classification tasks such as sentiment analysis, social meaning, topic, and dialect classification tasks and use learning rate $3$-$e^5$ on NER and QA tasks. 

\subsection{Experimental Results}
% #############################################
% Sentiment
% \input{evaluation/SA_res}
% \input{tables/tab_SA_res}
% \input{tables/tab_SA_acc.tex}


% ##################################
%  Social Meaning
% \input{evaluation/SM_res}
% \input{tables/tab_SM_res}
% ##############################################
% Topic Classification
% \input{evaluation/TC_res}
% \input{tables/tab_TC_res}

% ##############################################
% Dialect Identification
% \input{evaluation/DIA_res}
% \input{tables/tab_DIA_res}

% ##############################################
% NER
% \input{tables/tab_NER_res}
% \input{evaluation/NER_res}
% ##############################################
% QA
% \input{tables/tab_QA_res}
% \input{evaluation/QA_res}
% 
%
% 
% 
% 

==> evaluation/POS.tex <==
% \subsubsection{POS Results}

\noindent\textbf{Results.} \hl{to be added} As Table~\ref{tab:POS_res} shows, \ourmodel~outperform STOA on $3$ out of the $4$ datasets for POS. Indeed, \ourmodel~outperform the SOTA on EGY, LEV, and GULF with $+1.99\%$, $+0.89\%$, and $+0.15\%$ Accuracy, respectively. 

==> tables-App/tab_POS_res.tex <==
\begin{table}[]
\centering
\footnotesize
\begin{adjustbox}{width=0.9\columnwidth}
\begin{tabular}{lHcHlHHcc}
\toprule
 
               &       &      & \multicolumn{1}{c}{} & \multicolumn{2}{l}{~~~~\textbf{}} & \multicolumn{2}{l}{~~~~\textbf{TEST}} \\ 
               
               \cline{8-9} 
 
\multirow{-2}{*}{\textbf{Dataset (classes)}} &    & \multirow{-2}{*}{\textbf{SOTA}}& \multirow{-2}{*}{\textbf{Metric}} & \multirow{-2}{*}{\textbf{LM}}& \textbf{Acc.}              & \textbf{F$_1$}& \textbf{Acc.}              & \textbf{F$_1$} \\ \toprule
 &       &       &    & mBERT             & $92.51$	&$91.40$&	$92.68$	&$91.54$      \\
 &       &       &    & XLM-R\textsubscript{B}   & 00       & 00       & 00       & 00       \\
 &       &       &    & XLM-R\textsubscript{L}  & 00       & 00       & 00       & 00     \\
 &       &       &    & AraBERT           &$90.17$	&$89.60$&	$88.78$	&$89.14$       \\\cdashline{5-9}
 &       &       &    & \ourmodel         &  $91.38$&	$90.03$&	$90.23$	&$88.45$ \\
\multirow{-6}{*}{MSA } &          & \multirow{-6}{*}{\textbf{93.6}} & \multirow{-6}{*}{F1} & \newmodel           & $88.56$&	$86.31$&	$87.86$&	$85.71$\\\hline
 &       &       &    & mBERT             & $90.67$ &	$88.99$	 &$90.41$ &	$88.78$       \\
 &       &       &    & XLM-R\textsubscript{B}  &  00       & 00       & 00       & 00       \\
 &       &       &    & XLM-R\textsubscript{L} &  00       & 00       & 00       & 00     \\
 &       &       &    & AraBERT           &  $85.67$ &	$85.64$	 & $88.794$ &	$88.36$       \\\cdashline{5-9}
 &       &       &    & \ourmodel         &  $\textbf{93.67}$	 &$92.68$ &	$\textbf{93.05}$	  &$91.95$                \\
\multirow{-6}{*}{EGY}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{92.9}          & \multirow{-6}{*}{F1} & \newmodel           &  $91.67$	 &$89.77$ &	$89.53$ &	$87.91$ \\\hline
 &       &       &    & mBERT             &  $87.47$&	$84.47$&	$86.01$	&$82.79$      \\
 &       &       &    & XLM-R\textsubscript{B}  &  00       & 00       & 00       & 00     \\
 &       &       &    & XLM-R\textsubscript{L} &  00       & 00       & 00       & 00     \\
 &       &       &    & AraBERT           &  $82.95$&	$81.08$&	$83.89$	&$81.$       \\\cdashline{5-9}
 &       &       &    & \ourmodel         & $\textbf{89.77}$&	$87.51$	&$\textbf{88.88}$	&$86.42$ \\
\multirow{-6}{*}{LEV}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{87.9}  & \multirow{-6}{*}{F1} & \newmodel           &  $86.27$&	$83.18$&	$84.69$	&$80.89$ \\\hline
%  &       &       &    & mBERT             &  $\textbf{100.00}$&	$100.00$&	$\textbf{99.99}$	&$99.98$      \\
%  &       &       &    & XLM-R\textsubscript{B}  &  00       & 00       & 00       & 00       \\
%  &       &       &    & XLM-R\textsubscript{L} & 00       & 00       & 00       & 00     \\
%  &       &       &    & AraBERT           &  $98.42$	&$98.71$&	$97.89$&	$98.38$       \\\cdashline{5-9}
%  &       &       &    & \ourmodel         & $\textbf{100.00}$&	$100.00$&	$\textbf{99.99}$	&$99.99$       \\
% \multirow{-6}{*}{MAG}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{88.3}  & \multirow{-6}{*}{F1} & \newmodel           &$99.98$&	$99.97$	&$99.98$	&$99.97$ \\\hline





 &       &       &    & mBERT             &  $90.06$	&$87.47$&	$88.32$	&$85.04$       \\
 &       &       &    & XLM-R\textsubscript{B}  &    00       & 00       & 00       & 00   \\
 &       &       &    & XLM-R\textsubscript{L} &  00       & 00       & 00       & 00     \\
 &       &       &    & AraBERT           &  $83.08$	&$81.26$&	$85.48$	&$83.56$       \\\cdashline{5-9}
 &       &       &    & \ourmodel         & $\textbf{89.20}$	&$85.73$&	$\textbf{89.89}$&	$86.49$      \\
 \multirow{-6}{*}{GULF}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{87.9}  & \multirow{-6}{*}{F1} & \newmodel           & $88.53$	&$85.30$&	$89.46$	&$85.78$ \\\hline


\toprule

\end{tabular}
\end{adjustbox}
\caption{Performance of our models on POS task. SOTA results as reported in  ~\newcite{darwish2018multi}}
\label{tab:appedix_pos_res}
\end{table}

==> tables-App/tab_QA_res.tex <==

\begin{table}[ht]
\centering

\begin{adjustbox}{width=\columnwidth}
\begin{tabular}{lccclccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c}{\textbf{SOTA}}   &\multirow{2}{*}{~~~~\textbf{LM}} & \multicolumn{3}{c}{\textbf{TEST}}   \\ \cline{2-4} \cline{6-8} 
& \textbf{EM}  & \textbf{F$_1$}  &  \textbf{SM}   &  & \textbf{EM} & \textbf{F$_1$}  & \textbf{SM}   \\ \toprule
\multirow{4}{*}{ARCD}  & \multirow{4}{*}{{30.60\textsuperscript{$\star$}}} & \multirow{4}{*}{{62.70\textsuperscript{$\star$}}} & \multirow{4}{*}{{92.00\textsuperscript{$\star$}}} &      mBERT   &    \textbf{34.20} &  61.30  & 90.00   \\  
 &        &        &     &       AraBERT      & 30.60 & \textbf{62.70}   & \textbf{92.00}               \\  
  &     &         &       &        \ourmodel      & 31.76         & 61.64          & 88.88              \\ 
     &     &         &       & MARABERT   & 20.94         & 51.18          & 82.76                   \\                        
                                  
                                  \toprule

\multicolumn{8}{l}{\textsuperscript{$\star$}~\newcite{antoun2020arabert}}.
\end{tabular}
 \end{adjustbox}
\caption{\small{Performance of models on QA tasks.}}
\label{tab:appedix_QA_res}
\end{table}



==> tables-App/tab_SA_acc.tex <==
\begin{table}[]
\centering


\begin{adjustbox}{width=\columnwidth}
\renewcommand{\arraystretch}{1}{
\footnotesize
\begin{tabular}{lcHlccH} 
\toprule
\multirow{2}{*}{\textbf{Data (\#classes)} } & \multirow{2}{*}{\textbf{SOTA} }     & \multirow{2}{*}{\textbf{Metric} } & \multirow{2}{*}{\textbf{LM} } & \multicolumn{2}{l}{\textbf{~~~~~~TEST} }       \\ 
\cline{5-6}
&       &     & & \textbf{Acc.}        & \textbf{F1}          &   \\ 
\toprule

\multirow{6}{*}{AJGT (2)}     & \multirow{6}{*}{93.8\textsuperscript{$  $} }     & \multirow{6}{*}{Acc}& mBERT& 86.67  & 86.59  & 87.00      \\
&       &     &XLM-R$_{B}$       & 89.44  & 89.43  & 89.50      \\
&       &     & XLM-R$_{L}$      & 91.94  & 91.87  & 92.00      \\
&       &     & AraBERT         & 92.22  & 92.19  & 92.50      \\ \cdashline{3-6} 
&       &     &\ourmodel  & \textbf{94.44}       & 94.43  & 94.50      \\
&       &     & \newmodel& \textbf{96.11}       & 96.10  & 96.00      \\ 
\hline
\multirow{6}{*}{HARD (2)}     & \multirow{6}{*}{96.2\textsuperscript{$  $} }     & \multirow{6}{*}{Acc}& mBERT& 95.54  & 95.54  & 95.50      \\
&       &     &XLM-R$_{B}$       & 95.74  & 95.74  & 96.00      \\
&       &     & XLM-R$_{L}$      & 95.96  & 95.96  & 96.00      \\
&       &     & AraBERT         & 95.89  & 95.89  & 96.00      \\ \cdashline{3-6} 
&       &     &\ourmodel& \textbf{96.12}       & 96.12  & 96.00      \\
&       &     & \newmodel& \textbf{96.17}       & 96.17  & 96.00      \\ 
\hline
\multirow{6}{*}{ArsenTD-LEV (5)} & \multirow{6}{*}{59.4\textsuperscript{$  $} }     & \multirow{6}{*}{Acc}& mBERT& 50.50  & 47.98  & 51.50      \\
&       &     &XLM-R$_{B}$       & 55.25  & 49.89  & 57.00      \\
&       &     & XLM-R$_{L}$      & \textbf{62.00}       & 59.99  & 60.50      \\
&       &     & AraBERT         & 56.13  & 54.30  & 57.00      \\ \cdashline{3-6} 
&       &     &  \ourmodel& 61.38  & 58.06  & 62.00      \\
&       &     &  \newmodel& \textbf{60.38}       & 59.04  & 60.00      \\ 
\hline
\multirow{6}{*}{LABR (2)}     & \multirow{6}{*}{86.7\textsuperscript{$  $} }     & \multirow{6}{*}{Acc}& mBERT& 91.20  & 81.98  & 82.00      \\
&       &     &XLM-R$_{B}$       & 91.23  & 82.70  & 83.00      \\
&       &     & XLM-R$_{L}$      & 92.20  & 83.82  & 83.50      \\
&       &     & AraBERT         & 91.97  & 84.89  & 85.00      \\ \cdashline{3-6} 
&       &     & \ourmodel & \textbf{92.51}       & 84.98  & 85.00      \\ 
&       &     &  \newmodel & \textbf{92.49}       & 85.20  & 85.50      \\ 
\hline
\multirow{6}{*}{ASTD-B (2)} & \multirow{6}{*}{92.6\textsuperscript{$  $} }     & \multirow{6}{*}{Acc}              & mBERT        & 79.32 & 79.30 & 79.50   \\
          &    &  &XLM-R$_{B}$    & 87.59 & 87.55 & 87.50   \\
          &    &  & XLM-R$_{L}$   & 77.44 & 77.41 & 77.50   \\
          &    &  & AraBERT      & 83.08 & 83.07 & 83.50   \\ \cdashline{3-6} 
          &    &  & \ourmodel              & \textbf{93.23}       & 93.21 & 93.50   \\ 
          &    &  & \newmodel            & \textbf{96.24}       & 96.24 & 96.00   \\ 



\toprule

\multicolumn{6}{l}{ SOTA are results reported in \newcite{antoun2020arabert} based on Acc.}

\end{tabular}}\end{adjustbox}

\caption{\footnotesize{Performance of models on SA tasks (II).}}
\label{tab:appedix_senti_results_II}
\end{table}










==> tables/SA_corpus.tex <==
\footnotesize
\begin{center}
\begin{table*}[h]
\begin{tabular}   {p{3.4cm}cp{1.8 cm}p{1.1cm}cp{3.2cm}p{1.2cm}}

  \toprule
 \textbf{Authors }& \textbf{Task} & \textbf{Sources}&  \textbf{\# Data}  &\textbf{ Class } &\textbf{ Classes }    &\textbf{MSA/DI} \\
  \toprule
\newcite{abdul2012awatif} &   SSA & wikipedia,\textbf{\footnote{\textcolor[rgb]{0,0,1}{\url{https://www.wikipedia.com}}}} PAT,\textbf{\footnote{\textcolor[rgb]{0,0,1}{\url{https://catalog.ldc.upenn.edu/LDC2005T20}}}} Forums & $5,382$ &   4 & Obj,
Subj, Pos, Neg and Neut  & MSA  \\ %\hline
\newcite{abdulla2013arabic} &    SA & Twitter,  & $2000$ &   2& Pos, Neg & MSA \\ %\hline
\newcite{mageed2014samar} & SSA & Maktoob,\textbf{\footnote{\textcolor[rgb]{0,0,1}{\url{chat.mymaktoob.com}}}} Twitter & 11918 & 3 &   Obj,
Subj Pos, Subj Neg and Subj Mixed  & MSA+DI  \\ %\hline
\newcite{nabil2015astd} &    SSA & Twitter & $10000$ &   4 & Obj, Subj Pos, Subj Neg and Subj Mixed  & MSA \\ %\hline
\newcite{kiritchenko2016semeval}  &   SI &Twitter & $1,366$ & $-$ & Regression [0,1] & MSA\\ %\hline
\newcite{aly2013labr} &    SA & Book reviews & $63,000$ &   3& Pos, Neg, or Neut & MSA\\ %\hline
\newcite{salameh2015sentiment} &      SA   & BBN \textbf{\footnote{\textcolor[rgb]{0,0,1}{\url{ https://catalog.ldc.upenn.edu/LDC2012T09}}}}  & 1200 &   3 & Pos, Neg, or Neut & DI     \\ %\hline
\newcite{salameh2015sentiment} &      SA  & Twitter   & 2000 &   3 &  Pos, Neg, or Neut   & DI  \\ %\hline
\newcite{rosenthal2017semeval} &  SA &   Twitter&  9,500  &   2 &  Pos, or Neg  & MSA\\ %\hline
\newcite{rosenthal2017semeval} &   SA & Twitter &  3,400  &   3 & Pos, Neut, or Neg & MSA\\ %\hline
\newcite{rosenthal2017semeval} & SA & Twitter &  9,450  &  5  & High-Pos, Pos, Neut, Neg, Hihg-Neg & MSA\\ %\hline
\newcite{alomari2017arabic} &     SA & Twitter   & 1800 &   3 &Pos or Neg  & DI    \\ %\hline
\newcite{mohammad2018semeval} &  SA & Twitter & 1,800 &   7 & Various levels of Pos, Neg or Neut [-3,3]  & MSA\\ %\hline
Saad (2019)\textsuperscript{*}&   SA & Twitter &   58,751 &  2 &Pos, or Neg   & DI\\ %\hline
~\newcite{baly2019arsentd} &   SA &Twitter &  4,000 &   5& High-Pos, Pos, Neut, Neg, Hihg-Neg  & DI\\   \toprule
\end{tabular}
\caption{Sentiment analysis datasets. \textbf{SA}: Sentiment analysis.  \textbf{SSA}: Subjectivity and sentiment analysis. \textsuperscript{*}Dataset from Saad (2019) is available at \url{ https://www.kaggle.com/mksaad/arabic-sentiment-twitter-corpus}.}
\label{tab:sentiment}
\end{table*}
\end{center}

\normalsize 

==> tables/SM_tasks.tex <==
\footnotesize
\begin{center}
\begin{table*}[ht]
\begin{tabular}   {p{3.7cm}cp{1.7 cm}p{1.1cm}cp{2.4cm}p{1.2cm}}

  \toprule
 \textbf{Authors }& \textbf{Task} & \textbf{Sources}&  \textbf{Data}  &\textbf{ Class } &\textbf{ Classes }    &\textbf{MSA/DI} \\
  \toprule

\newcite{alshehri2020understanding} &      Dangerous  & Twitter   & $4,445$ &   2 &  safe or not & MSA+DI  \\ %\hline
\newcite{al2020proceedings} &  Offensive &   Twitter& $10,000$  &   2 &  offensive or not  & MSA+DI\\ %\hline
\newcite{al2020proceedings} &   Hate & Twitter &  $10,000$   &   2 & hate or not & MSA+DI\\ %\hline
\newcite{farha2020arabic} & Sarcasm & Twitter &  $10,575$  &  2  & sarcasm or not& MSA+DI \\ %\hline
\newcite{farha2020arabic} & DI* & Twitter &  $10,575$  &  5  & sarcasm or not& MSA+DI \\ %\hline
\newcite{farha2020arabic} & SA* & Twitter &  $10,575$  & 3  & sarcasm or not& MSA+DI \\ %\hline
  \toprule
\end{tabular}
\caption{Social Meaning Tasks Datasets. }
\label{tab:sentiment}
\end{table*}
\end{center}
\normalsize 


==> tables/tab_POS_res.tex <==
\begin{table}[]
\centering
\footnotesize
\begin{adjustbox}{width=0.9\columnwidth}
\begin{tabular}{lHcHlHHcc}
\toprule
 
               &       &      & \multicolumn{1}{c}{} & \multicolumn{2}{l}{~~~~\textbf{}} & \multicolumn{2}{l}{~~~~\textbf{TEST}} \\ 
               
               \cline{8-9} 
 
\multirow{-2}{*}{\textbf{Dataset (classes)}} &    & \multirow{-2}{*}{\textbf{SOTA}}& \multirow{-2}{*}{\textbf{Metric}} & \multirow{-2}{*}{\textbf{LM}}& \textbf{Acc.}              & \textbf{F$_1$}& \textbf{Acc.}              & \textbf{F$_1$} \\ \toprule


 &       &       &    & mBERT             & $92.51$	&$91.40$&	$92.68$	&$91.54$      \\
 &       &       &    & XLM-R\textsubscript{B}   & $95.44$&	$94.78$&	$93.29$	&$92.55$       \\
 &       &       &    & XLM-R\textsubscript{L}  & $97.16$	&$\bf96.79$&	$\bf96.85$&$96.24$     \\
 &       &       &    & AraBERT           &$90.17$	&$89.60$&	$88.78$	&$89.14$       \\\cdashline{5-9}
 &       &       &    & \ourmodel         &  $91.38$&	$90.03$&	$90.23$	&$88.45$ \\
\multirow{-6}{*}{MSA } &          & \multirow{-6}{*}{93.6} & \multirow{-6}{*}{F1} & \newmodel           & $88.56$&	$86.31$&	$87.86$&	$85.71$\\\hline
 &       &       &    & mBERT             & $90.67$ &	$88.99$	 &$90.41$ &	$88.78$       \\
 

 &       &       &    & XLM-R\textsubscript{B}  &  $92.16$&	$91.00$&	$91.84$&	$90.42$       \\
 &       &       &    & XLM-R\textsubscript{L} &  $\bf96.54$	&$95.95$&	$\bf96.06$	&$95.34$     \\
 &       &       &    & AraBERT           &  $85.67$ &	$85.64$	 & $88.794$ &	$88.36$       \\\cdashline{5-9}
 &       &       &    & \ourmodel         &  $93.67$	 &$92.68$ &	$93.05$	  &$91.95$                \\
\multirow{-6}{*}{EGY}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{92.9}          & \multirow{-6}{*}{F1} & \newmodel           &  $91.67$	 &$89.77$ &	$89.53$ &	$87.91$ \\\hline
 &       &       &    & mBERT             &  $87.47$&	$84.47$&	$86.01$	&$82.79$      \\


 &       &       &    & XLM-R\textsubscript{B}  &  $83.71$	& $80.67$	& $84.90$	& $81.29$     \\
 &       &       &    & XLM-R\textsubscript{L} &  $\bf92.98$	& $91.38$	& $\bf91.28$	& $89.58$    \\
 &       &       &    & AraBERT           &  $82.95$&	$81.08$&	$83.89$	&$81.64$       \\\cdashline{5-9}
 &       &       &    & \ourmodel         & $89.77$&	$87.51$	&$88.88$	&$86.42$ \\
\multirow{-6}{*}{LEV}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{87.9}  & \multirow{-6}{*}{F1} & \newmodel           &  $86.27$&	$83.18$&	$84.69$	&$80.89$ \\\hline
%  &       &       &    & mBERT             &  $\textbf{100.00}$&	$100.00$&	$\textbf{99.99}$	&$99.98$      \\
%  &       &       &    & XLM-R\textsubscript{B}  &  00       & 00       & 00       & 00       \\
%  &       &       &    & XLM-R\textsubscript{L} & 00       & 00       & 00       & 00     \\
%  &       &       &    & AraBERT           &  $98.42$	&$98.71$&	$97.89$&	$98.38$       \\\cdashline{5-9}
%  &       &       &    & \ourmodel         & $\textbf{100.00}$&	$100.00$&	$\textbf{99.99}$	&$99.99$       \\
% \multirow{-6}{*}{MAG}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{88.3}  & \multirow{-6}{*}{F1} & \newmodel           &$99.98$&	$99.97$	&$99.98$	&$99.97$ \\\hline






 &       &       &    & mBERT             &  $90.06$	&$87.47$&	$88.32$	&$85.04$       \\
 &       &       &    & XLM-R\textsubscript{B}  &    $88.12$	&$85.39$&	$89.10$&	$85.79$  \\
 &       &       &    & XLM-R\textsubscript{L} &  $\bf90.92$	&$89.16$&	$\bf91.20$&	$88.80$     \\
 &       &       &    & AraBERT           &  $83.08$	&$81.26$&	$85.48$	&$83.56$       \\\cdashline{5-9}
 &       &       &    & \ourmodel         & $89.20$	&$85.73$&	$89.89$&	$86.49$      \\
 \multirow{-6}{*}{GULF}  & \multirow{-6}{*}{---}              & \multirow{-6}{*}{87.9}  & \multirow{-6}{*}{F1} & \newmodel           & $88.53$	&$85.30$&	$89.46$	&$85.78$ \\\hline


\toprule

\end{tabular}
\end{adjustbox}
\caption{Performance of our models on POS task. SOTA results as reported in  ~\newcite{darwish2018multi}}
\label{tab:POS_res}
\end{table}

==> tasks/POS.tex <==
\subsection{Part-Of-Speech  Tagging} \label{sec:tasks_TC}
POS tagging is a token-level classification task, which consists of assigning each word in a given sentence its corresponding grammatical category \cite{ habash-2010,darwish2017arabic}.   We next introduce briefly the datasets used in this task. 


% \subsubsection{Datasets}

\noindent\textbf{Datasets.} In order to investigate our models on this task, we fine our models on a multi-dialect Arabic POS tagging datasets proposed by ~\newcite{darwish2018multi} which covers  MSA (with $18$ POS tag) and four in dialects (tweets) EGY, MAG, LEV, and GOLF. The MSA data has $18$ POS  tag  described  by \newcite{darwish2017arabic}. For the dialects  ~\newcite{darwish2018multi} added $2$  dialect-specific  tags (\textit{progressive part and  negation part})  and  4  tweet-specific  tags  (\textit{hash,emoticon/emoji, mention, and URL}).  Table~\ref{tab:POSdata}   provide a description summary of 5 datasets.

% #######################################################
\begin{table}[ht]
\centering
\ \footnotesize
\begin{tabular}{lrrrr}
\hline

\textbf{Dataset(class.)} & \textbf{Tokens}          & \textbf{TRAIN}   & \textbf{DEV} & \textbf{TEST}             \\ \hline 
% AQC-MSA    & $150K$ & $6,504$ & $5,018$ & $3,437$ \\ 
MSA (18) & $25.5$K & $17.9$K  & $5.3$K & $2.5$K  \\

LEV (24) & $22.7$K &$16.4$K & $2.2$K & $4.3$K  \\

EGY (24) & $23.6$K & $17.4$K & $1.9$K & $4.7$K \\ 

% MAG  (24)   & $101.1K$ & $71.1$K & $9.8$K & $20.2$K  \\ 


GULF (24)     & $20.9K$ & $14.7$K & $2.2$K & $4.3$K  \\ \cdashline{1-5}

\textbf{ArBench\textsubscript{POS}} & $92.7$K & $65.6$K & $8.7$K & $18.6$K \\  
\toprule
\end{tabular}
\caption{Distribution of classes and token size of the Arabic POS datasets~\cite{darwish2018multi}.}
\label{tab:POSdata}
\end{table}
% #######################################################

%-----------------------


%-----------------------
% \subsubsection{Baselines}
%-----------------------
\noindent\textbf{Baselines.} \hl{We  compare  our  results  with  the STOA as reported by}~\newcite{darwish2018multi}. They use CRF sequence labeler to build the POS tagger using clitic n-gram features, stem templates, and clitic
metatypes.They report the best accuracy using the combined features as $93.6$, $92.9$, $87.8$, $87.8$ for MSA, EGY, LEV,and GLF respectively.  

\input{tables/tab_POS_res}
\input{evaluation/POS}
